Is Private Learning Possible with Instance Encoding?

A private machine learning algorithm hides as much as possible about its training data while still preserving accuracy. In this work, we study whether a non-private learning algorithm can be made private by relying on an instance-encoding mechanism that modifies the training inputs before feeding them to a normal learner. We formalize both the notion of instance encoding and its privacy by providing two attack models. We first prove impossibility results for achieving a (stronger) model. Next, we demonstrate practical attacks in the second (weaker) attack model on InstaHide, a recent proposal by Huang, Song, Li and Arora [ICML'20] that aims to use instance encoding for privacy.

==> 08_old_overview.tex <==
\section{Overview of Theoretical Barriers}
\label{sec:barriers}


\subsection{Our Results} We prove several theoretical barriers for (carefully defined notions of) privacy of encoding-based learning mechanisms. Our first barrier is proved for \emph{dataset} encoding schemes, while  our second barrier is proved for \emph{instance} encoding schemes. In Section~\ref{sec:instahide_attack} we also show an algorithm that achieves a successful \emph{reconstruction} on the recent InstaHide protocol of  \cite{huang2020instahide}, which relies on instance encoding. However, the focus of this section is to highlight the general theoretical barriers.

\paragraph{Limits of privacy with dataset encoding.} We first study \emph{distinguishing} attacks whose goal is to find out with probability (non-negligibly) more than $\sfrac12$ which dataset out of $S_1,S_2$ has been randomly chosen and encoded. In fact, we will show how to achieve this even if the datasets share many similarities and only differ in one example pair (with the same label).
%\SJ{I am assuming anything above $50\%$ will be fine. Right? If so, we should say it. Also, we should say the restriction
%on the concept classes is not a big deal. Most reasonable concept classes will have that.} \Mnote{I added it.}
\begin{theorem}[Informally stated -- limits of privacy based on dataset encoding] \label{thm:Inf1} Let $(E,L)$ be an arbitrary encoding and learning scheme with  at least $70\%$ accuracy on the original data (not the encoded data).
%Suppose the class of the concept functions is rich enough as follows. There are two concept functions $c_1,c_2$ that are both balanced and are orthogonal over the uniform distribution. Suppose we want to learn all four functions $C=\set{c_1,c_2,1-c_1,1-c_2}$. Then there is an adversary who can construct two datasets $S_1,S_2$ and pick $c \gets C$ such that:
Then for any ``nontrivial'' concept class $C$ (e.g., sufficient to be closed under complement and to contain at least two distinct concepts), there is an adversary who can pick datasets $S_1,S_2$ and pick a concept $c \gets C$ and distinguish their encodings with probability $1/2 + \Omega(1/n)$, while the sets satisfy the following restrictions:
\begin{enumerate}
    \item All instances in $S_1,S_2$ are cleanly labeled (by  $c$).
    \item $S_1=\set{e_1}\cup S,S_2=\set{e_2}\cup S$ differ in one sample only.
    \item The differing examples $e_1=(x_1,y),e_2=(x_2,y)$  still have the same label $y$ (i.e., $c(x_1)=c(x_2)=y$).
\end{enumerate} 

\end{theorem}

\paragraph{Discussion.} Theorem~\ref{thm:Inf1} gives a \emph{distinguishing} attack of advantage $\Omega(1/n)$. Moreover, since the two datasets used by the adversary are neighbors (i.e., differ in one point), this also implies a lower bound on the sample complexity of differentially private learners (based on the given $\eps$ parameter of the differential privacy). This result further shows that none of the restrictions on the adversary (as stated in Theorem~\ref{thm:Inf1}) can enable a way to limit the adversary's distinguishing advantage (or the corresponding $\eps$ in a candidate differentially private scheme) to $o(1/n)$. In fact, the actual proof of Theorem~\ref{thm:Inf1} proves something stronger: the adversary will \emph{not} pick the core  set $S$ that is shared between $S_1,S_2$, but rather that set is \emph{sampled} from a distribution that is specified by the adversary. Finally we note that the complexity of the concept functions in Theorem \ref{thm:Inf1} cannot be reduced to having only one concept function. That is because, if $C=\set{c}$, the learner can basically ignore the data and just output a canonical representation of $c$, leading to a perfectly private scheme.
%This distribution $\cD$, however, is still dominated by the uniform distribution over $X$, which means that when $X$ is superpolynoially large, the adversary basically knows none of the samples in $S$.

\paragraph{Related work.} As mentioned above,  Theorem~\ref{thm:Inf1}  can be seen as a  (dimension-independent) lower bound on the sample complexity of (even differentially private) PAC learning.  Some previous work have studied similar lower bounds on sample complexity of learning algorithms in various contexts. For example the prior works of~\cite{duchi2014local,hardt2010geometry, bun2016order} used a  packing argument to give sharp bounds for  parameter/probability
estimation goals, and the work of~\cite{bun2018fingerprinting} proves lower bounds on the sample complexity of differentially private algorithms that accurately answer large sets of counting queries. In addition, lower bounds on the sample complexity of  differentially private (general) PAC learning were proved in \cite{bassily2014private,beimel2014bounds}. It might be possible to improve Theorem~\ref{thm:Inf1} by incorporating the data dimension, however not depending on the dimension is a postive, and we emphasize that our result comes with specific guarantees that are important: the two sets are consistent with a concept function and have the same set of labels. This makes our lower bound more amenable to real world setting, where we want to distinguish two data sets with say, the same number of cat and dog images in them.

\paragraph{Limits of privacy with instance encoding.} We now describe our next result which states the limits of what \emph{instance} encoding (as a special form of general dataset encoding) can offer for (our minimal and natural indistinguishability-based notion of) data privacy. In this setting, we deal with a \emph{decomposable} encoding, which encodes instances and their labels separately. Such decomposable encodings can cover, e.g., the mix-up operation \cite{zhang2017mixup} used in InstaHide \cite{huang2020instahide}. For encoding $\tilde{x}$ and instance $x$, we write $x \in E^{-1}_X(\tilde{x})$ if $x$ is one of the instances that are used for generating the encoding $\tilde{x}$.

One natural property that an instance encoding mechanism can provide is to enable the trained model to have some (perhaps weak) form of accuracy in predicting labels on the  \emph{encoded data}. For example, suppose $x$ is used, as one of the $r$ instances in a $r$-local instance encoding mechanism (defined by an encoded sample $\tilde{x}$ depending on $r$ distinct training samples), then we could ask the trained model $h$ to  predict the \emph{true} concept $c(x)$ of $x$ on the encoded sample $\tilde{x}$ as well. 
Indeed, we define (see Definition~\ref{def:accuracyEnc}) the  notion of \emph{encoded accuracy} for the model  $h$ to be  the probability of satisfying $h(\tilde{x})=c(x))$ when $x$ is a random instance and $x \in E^{-1}_X(\tilde{x})$. Of course this notion of accuracy may only be satisfiable in a \emph{weak} sense, as each locally encoded instance $\tilde{x}$ depends on $r$ different examples which may have different labels.
However, we argue that natural instance encoding schemes could still allow the error to be bounded away from (and smaller than) $1/2$. For example, using a $2$-local encoding on all pairs $(x,x')$ of instances in a set $S$ potentially allows  getting (weak) accuracy on encoded instances of $\approx 0.75$, because when the labels of $(x,x')$ are the same, the prediction of the model $h$ on the encoded string $\tilde{x}$ could be close to $1$, and in other cases it could be close to $0.5$. 

In our next result we show barriers for achieving privacy based on instance encoding, when two conditions hold: (1) The goal of the adversary is to distinguish encodings $\tilde{x}$ where $x \in E^{-1}_X(\tilde{x})$ from those where $x' \in E^{-1}_X(\tilde{x})$ for $x \neq x'$. (2) The learning protocol $(E,L)$ allows some nontrivial accuracy on \emph{encoded} strings as defined above.
%\SJ{Is influenced the right term there?} \Mnote{I removed the term and substituted it with a mathematical notation.}

\begin{theorem}[Informally stated -- limits of privacy based on instance encoding] \label{thm:Inf2}
Suppose the goal is to learn instances that are distributed according to distribution $\cD$ and  the concept class is rich enough to contain $m$ concept functions $c_1,\dots,c_m$ that are each balanced under $\cD$ and are also independent from each other. (For example, this would be the case when the concepts contain $m$ orthogonal half spaces in dimension $m$ and $\cD$ is the isotropic Gaussian in the same dimension $m$). Also, suppose the protocol $(E,L)$ has \emph{encoded} accuracy $1/2 + \delta$ for a constant $\delta > 0$ (that can depend on the locality of $E$, e.g., $\delta\approx2^{-r}$). Then, the adversary can distinguish the encodings of two randomly selected instances $x,x' \gets D$ with advantage $\Omega(1)$ (over the trivial bound of $1/2$).
\end{theorem}

We also prove a variant of Theorem \ref{thm:Inf2} in which we do \emph{rely} on the richness of the concept class, but instead we obtain a weaker guarantee that \emph{either} of the following happens: either (1) we obtain a distinguishing attack on the instance encoding, or (2) we show that the learning error on original instances can be arbitrarily close to $0$. This barrier applies to any setting where state-of-the-art classifiers achieve accuracy bounded away (by some constant) from $1$ (e.g., image classification). 
%\Mnote{what is the citation for SOTA image classification errors?}\nicholas{I think it's just saying it's true for any classifier that's not perfect?}

\paragraph{Further related work.} For the details of our reconstruction attack on InstaHide we refer the reader to Section \ref{sec:instahide_attack}. Here we mention some related work. Our attacks on data privacy of ML models are related to ``membership inference'' attacks~\cite{shokri2017membership,long2017towards,salem2019ml,long2018understanding,yang2019neural} as well as  \emph{model inversion} attacks \cite{fredrikson2014privacy,fredrikson2015model,wu2016methodology,VBE18}, and our attack on InstaHide is a form of reconstruction attack
\cite{dinur2003revealing,dwork2017exposed,backes2016membership,dwork2015robust,sankararaman2009genomic,homer2008resolving}.


%\Mnote{Here It looks like we are saying that the argument of previous paragraphs does not apply... I tried to reword it but still looks something that might be improvable.}

%As mentioned earlier, this attack is not as strong. Thus, we focus on weaker notions of security/privacy and provide more devastating attacks.  \FT{What do we mean by this last paragraph?}
\setcounter{theorem}{0}

%See the technical overview section below for the sketch of the ideas behind the proof of Theorem~\ref{thm:Inf2}

\subsection{Technical Overview of Theoretical Barriers}
Here we sketch the key ideas for proving Theorems~\ref{thm:Inf1} and~\ref{thm:Inf2}.

\paragraph{Ideas behind the proof of Theorem~\ref{thm:Inf1}.}
As a first step, we show show how to achieve the goals of Theorem~\ref{thm:Inf1} by  dropping the first two conditions, and then we will show how to additionally achieve those conditions. Let $c_1 \in C$ be a concept function, and let $c'_1=1-c_1\in C$ be the complement function that flips the labels, and assume $1-c_1 \in C$ as well. Let $S_1$ (resp. $S_2$) be  a dataset of size $n$ that is obtained by uniformly and independently sampling $n$ instances from $X$ and labeling them according to $c_1$ (resp. $c_1'$). If the adversary receives one of the encodings $E(S_1),E(S_2)$ chosen at random by a challenger, it can find out which one is selected by running the learning $L$ algorithm over the given encoding $\tilde{S}$ first to obtain a model $h \gets L(\tilde{S})$. It then asks a query $x \gets X$ to $h$ and obtains $h(x)$, and then it will compare the answer to both of $c_1(x),c'(x)$. Since the learning algorithm is supposed to learn effectively, this simple attack will be successful in distinguishing the two encodings.

One catch in the argument above is that the challenge sets $S_1,S_2$ are generated with respect to  \emph{two} concept functions. This means that the training sets are somehow of ``different nature'', and so it might not be surprising that their encoding is distinguishable. Another catch is that the datasets are almost completely separate (and do not \emph{share} $n-1$ examples  -- in fact they \emph{cannot} share \emph{any} examples when they use complementary concepts). Our main idea comes to help for showing how to resolve the first issue by taking advantage of the richness of the concept class    as follows. Suppose $c_2$ is another concept  function that is independent and in fact orthogonal to $c_1$ (and so  $1-c_1$ as well). For example, $c_1$ could be the concept of cat versus dog, and $c_2$ could be the concept of having long hair versus short hair. Such $c_2$ will partially agree with $c_1$ (over a subset of $X$) and $1-c_1$ both. The key idea is that since the adversary can distinguish $c_1$ from $c_2$, it should also be able to distinguish either samples chosen from $c_1$ from those of $c_2$, or it should achieve this between $c'_1,c_2$. This is indeed a hybrid argument. This is not still enough, as we want the samples in each of these cases to be selected from points that both concepts \emph{agree} on the answers. Doing so will allow the adversary to ``confuse'' the encoding scheme (because it will not know which concept is being used) and switch the concept function to another one (so long as we only sample instances over which they have the same answers). To make sure about such consistency, we can also change the distribution $\cD$ (form which we sample the instances) from being completely uniform to being uniform over subsets that the concepts $c_1,c_2$ agree or disagree. By designing such hybrids carefully, we can conclude that there is a concept $c \in \set {c_1,1-c_1,c_2} $ that can be used to label \emph{both} sets $S_1,S_2$ while the adversary will distinguish their encodings with advantage $\Omega(1)$. 

The above trick resolves the first issue (and gives us  Item 1 of Theorem~\ref{thm:Inf1}), but it still uses different distributions in different hybrids, and so the sampled sets would be almost completely disjoint. To satisfy Item 2 of Theorem~\ref{thm:Inf1} we make further use of hybrids that gradually and carefully change the distributions in such a way that the statistical distance between the two distributions would be (almost) $1/n$. This  way, the adversary can use the single instance that make $S_1,S_2$ different, and let the rest of $S_1,S_2$ be sampled identically. See Section \ref{sec:impossibilities} for the formal statement and Appendix~\ref{apx:proof1} for the proof. %\Mnote{If proofs are going to be in the appendix, we need to give pointers to them here.}

%We consider $3$ hybrids between the two worlds in which $c_1$ (hybrid 0) or $1-c_1$ (world 4) are used for labelling the instances. Suppose $c_1$ is balanced, and $c_2$ is another balanced function that is orthogonal to $c_1$; namely, for any $(b_1,b_2) \in \bits^n$, we have that $Pr_{x \gets U_X}[c_1(x)=b_1 \land c_2(x)=b_2]=1/4$. The middle hybrid 2 will use concept function $c_2$

\paragraph{Ideas behind the proof of Theorem~\ref{thm:Inf2}.} In a nutshell, the idea behind the proof of Theorem~\ref{thm:Inf2} is as follows. Having non-trivial accuracy of predicting the labels of the instances used in an encoding by only looking at the encodings (i.e., having encoded accuracy as defined above) we are in fact allowing the learning process to produce a ``key'' $h$ that allows us to \emph{practically decode} the hidden label of the original instance $x$ by looking at the encoding $\tilde{x}$. This already constitutes a nontrivial information whose leakage could be leveraged for launching a distinguishing attack between various encodings. To amplify the confidence, this trick could be used multiple times using various concept functions $c_1,\dots,c_m$ as fingerprints that tell us how to distinguish the instances behind the encodings.

More formally,  let $F=(c_1,c_2,\dots,c_m)$ be  $m$ concept functions all from $C$ that are (1) balanced  and (2) orthogonal under $\cD$. These two conditions imply that $F(x)$ for a random $x \gets D$ is a uniformly distributed Boolean vector of dimension $m$ (i.e., $\Pr[F(D)=f]=2^{-m}$ for any $f \in \bits^m$) and hence, by standard concentration bounds, the Hamming distance of $F(D)$ from any fixed Boolean vector $f \in \bits^m$ is be concentrated around $m/2$. Moreover,  the adversary can use samples form $\cD$ and oracle access to concepts $c_1,\dots,c_m$ to train models $h_1,\dots,h_m$ that approximate $c_1,\dots,c_m$ \emph{on encoded strings}. (The latter is due to the presumed encoded accuracy property). Now, suppose the adversary  knows that a given encoded value $\tilde{x}$ is  based on some $x \in \set{x_1,x_2}$, and it wants to find out which instance is indeed used for the encoding. Then, the adversary can use the trained models $h_1,\dots,h_m$ to get a noisy fingerprint $f'$ of $F(x)=f$ that still has (slightly) more than half of the coordinates right (i.e., Hamming distance of $f'$ and $f$ is less than $m/2$). On the other hand, if both challenges $\set{x_1,x_2}$ are chosen at random, and if we let $x' \in \set{x_1,x_2}$ be the ``other'' instance that is not used in the encoding,  then the Hamming distance between $F(x')$ and $f'$, with high probability, would be  $(1\pm o(1)) \cdot m/2$. As a result, by comparing $f'$ with both of $F(x_1)$ and $F(x_2)$, and picking $x_b$ that minimizes the Hamming distance between $f'$ and $F(x_b)$, the adversary can find out the right answer. See Section~\ref{sec:impossibilities} for the formal statement and Appendix~\ref{apx:proof2} for the full proof.

\subsection{Key Ideas of Our Concrete Attack (and connections to theory)}
